MIRROR: Differentiable Deep Social Projection for Assistive Human-Robot Communication

Communication is a hallmark of intelligence. In this work, we present MIRROR, an approach to (i) quickly learn human models from human demonstrations, and (ii) use the models for subsequent communication planning in assistive shared-control settings. MIRROR is inspired by social projection theory, which hypothesizes that humans use self-models to understand others. Likewise, MIRROR leverages self-models learned using reinforcement learning to bootstrap human modeling. Experiments with simulated humans show that this approach leads to rapid learning and more robust models compared to existing behavioral cloning and state-of-the-art imitation learning methods. We also present a human-subject study using the CARLA simulator which shows that (i) MIRROR is able to scale to complex domains with high-dimensional observations and complicated world physics and (ii) provides effective assistive communication that enabled participants to drive more safely in adverse weather conditions.

==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}
discussion comes here

\hsnote{need some key takeaways:}

while not explored in this work, we could also use the same MIRRoR model to communicate actions, e.g., ``\textsf{Turn Right}'', rather than information about cars in the environment. 
depends on similarity between the human and the robot self-model. drastic differences will of course render the self-model to be not a useful reference point. 

social projection to social behavior? Can the model be used to improve cooperation? 

use for explanation and not only communication. 

\hsnote{limitations is unidentifiability. whether the difference in the policy or the perception cannot be completely ascertained (?). Future work can look into methods that resolve this ambiguity, e.g., keeping a distribution over parameters [REF] or via bayesian optimization [REF] similar to IRL scenarios.}
\hsnote{mirror cannot handle cases where the human observes more than the robot.}

